Cost-to-Go Function Generating Networks for High Dimensional Motion Planning

This paper presents c2g-HOF networks which learn to generate cost-to-go functions for manipulator motion planning. The c2g-HOF architecture consists of a cost-to-go function over the configuration space represented as a neural network (c2g-network) as well as a Higher Order Function (HOF) network which outputs the weights of the c2g-network for a given input workspace. Both networks are trained end-to-end in a supervised fashion using costs computed from traditional motion planners. Once trained, c2g-HOF can generate a smooth and continuous cost-to-go function directly from workspace sensor inputs (represented as a point cloud in 3D or an image in 2D). At inference time, the weights of the c2g-network are computed very efficiently and near-optimal trajectories are generated by simply following the gradient of the cost-to-go function. We compare c2g-HOF with traditional planning algorithms for various robots and planning scenarios. The experimental results indicate that planning with c2g-HOF is significantly faster than other motion planning algorithms, resulting in orders of magnitude improvement when including collision checking. Furthermore, despite being trained from sparsely sampled trajectories in configuration space, c2g-HOF generalizes to generate smoother, and often lower cost, trajectories. We demonstrate cost-to-go based planning on a 7 DoF manipulator arm where motion planning in a complex workspace requires only 0.13 seconds for the entire trajectory.

==> inline_todonotes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following makes inline todonotes behave nicely
\usepackage{todonotes,varwidth}
\makeatletter
\tikzstyle{diaanotestyle} = [
    draw=\@todonotes@currentbordercolor,
    fill=\@todonotes@currentbackgroundcolor,
    line width=0.5pt,
    inner sep = 0.8 ex,
    rounded corners=4pt,align=left,
   ]

\renewcommand{\@todonotes@drawInlineNote}{%
        {\begin{tikzpicture}[remember picture,baseline={(0,0)}]%
            \draw node[diaanotestyle,font=\@todonotes@sizecommand,anchor=base west]{%
               \begin{varwidth}[t]{5cm}
                \if@todonotes@authorgiven%
                    {\@todonotes@sizecommand \@todonotes@author:\,\@todonotes@text}%
                \else%
                    {\@todonotes@sizecommand \@todonotes@text}%
                \fi
                \end{varwidth}};%
            \end{tikzpicture}}%
       }%
\makeatother   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> intro_old.tex <==

\section{Introduction}  
%
Planning for robotic manipulation is one of fundamental and essential problems in robotics since planning performance is a key factor for the performance of robot systems. Although many approaches has been extensively studied to develop efficient and fast planning approaches, planning for manipulators with obstacle avoidance is cumbersome since it requires extensive collision checking with kinematics and considerable iterative propagation of cost values. In DARPA robotic challenges, many robots show slow performance and failures for manipulation tasks \cite{spenko2018darpa}. 

Although search based planning such as A* and Dijkstra \cite{bonet2001planning,maximARA,stentz1995focussed} can find the optimal trajectory for target goals in low dimensional space rapidly, they are not applicable for planning of many degree of freedoms (dof) manipulators due to curse of dimensionality in high-dimensional space. There are sampling sampling based planners such as Probabilistic Roadmaps (PRM) or Rapidly Exploring Random Trees (RRT) planners \cite{lavalle2006planning,kavraki1996probabilistic,karaman2011anytime, gammell2014informed, bekris2003multiple,urmson2003approaches,jaillet2010sampling,conner_rizzi_choset_IROS2003}, They are also degraded in high dimensional space due to requiring many samples and collision check routines. 

In this paper, we propose a neural network approach for generating a continuous \ctog{} function in configuration space of manipulator given information in workspace such as images, voxels, or pointclouds. Specifically, we present a Higher Order Function (HOF) network~\cite {mitchell2019higher,wang2020geodesic}. We train a HOF to learn to output the \ctog{} function over the \cmap.  Both the HOF and the \ctog{} function are represented as neural networks and it can generate a continuous trajectory by following the gradient of this \ctog{} function.




Although we investigated the feasibility of c2g-HOF in \cite{}, the input of HOF is C-space map representing of collision region in C-space in the prior work. In addition, since it use two dimensional or three dimensional convolution layers for c-space map, it has limitation for applying for high-dimensional space. It also uses one fixed goal configuration. 

Compared to prior work, our method provides an enhanced framework that includes PointNet \cite{qi2017pointnet} with 3D pointcloud of obstacles in workspace instead of convolution of C-sapce map; thus it encodes any obstacle status immediately with a high dof manipulator and it is applicable for motion planning in high-dimensional C-space. In addition, since the \ctog{} function network is learned to estimate a \ctog{} value, the planner plans for any target configurations.
%
\begin{figure}[]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/c2g_hof_overview.png}
    \caption{System Overview. During training, we train the network with cost-to-go values from Dijkstra or PRMs but we use only c2g-HOF network for inference.}
    \label{fig:overview_flowchart}
\end{figure}


% HERE HERE
As shown in Fig. \ref{fig:overview_flowchart}, The c2g-HOF then generates the cost-to-go function for a given pointcloud in workspace. The HOF network generates the weights of the neural network representing the cost-to-go as a smooth and continuous function. HOF is trained with ground truth cost-to-go values computed by Dijkstra or PRM.
The motion plan can be generated by following the gradient of the output cost-to-go function. 
The main advantage of our method is that, once trained, it can instantly generate a continuous cost-to-go map with one target configuration over the entire C-map much faster than other approaches. 

In summary, the core contributions of the paper include 1) c2g-HOF generating continuous \ctog function networks without discretization, considerable iterative propagation of cost values, and extensive collision checks, 2) Efficient planning based on \ctog function network in \cspace given pointcloud in workspace for a target configuration, 3) Design of c2g-HOF networks applicable for high-dimensional C-space of manipulator. It allows for motion planning in high degree-of-freedom manipulators to be much faster compared to previous planning algorithms.


==> problem_old.tex <==

\subsection{Problem Definition}

%We consider a setup which consists of a manipulator and an external sensor to measure obstacles in workspace $\mathcal{W}$. In this setup, given a robot with a configuration space $\mathcal{C}$ corresponding to $\mathcal{W}$, 

Let $f_{\mathcal{W}}: \mathcal{C}  \times \mathcal{C}  \rightarrow
[0, \infty)$
%\mathbb{R}^+ \cup \{0\}$ 
be the cost to go function which, for any given $s, t$ in the configuration space $\mathcal{C}$ returns the cost to traverse a piecewise collision-free smooth curve from $s$ to $t$. 
%$\mathbb {C} \subset \mathcal {C}$.


The objective is to train a neural network which outputs $f_{\mathcal{W}}$ from input $\mathcal{W}$.


Our method requires a representation of the workspace $\mathcal{W}$ as input. In this paper, we consider two such representations which cover a large number of application scenarios: (i)~3D obstacles represented as a point cloud, and (ii)~an overhead depth image of a 2.5D workspace. 

During training, we assume that a planner which can  compute the cost-to-go between two configurations is available. The specific metric used for computing the cost (e.g. length or energy) is determined by the planner.


% We also assume that the robot kinematics are given, and that collisions in the configuration space $\mathcal{C}$ can be determined.




% learn a cost-to-go function $f_{\mathcal{W}}(s, t)$ in $\mathcal{C}$ where $f_{\mathcal{W}}(s, t)$ is a \ctog value in \cspace between two configurations $s$ and $t$, $s, t \in \mathcal{C}$. The cost-to-go value between $s$ and $t$ is the integral of distance along a piecewise collision-free smooth curve $\mathbb {C} \subset \mathcal {C}$. %and $\mathbb {C}$ is defined by any trajectory generation planners. 

% During training, we assume that a planner which can  compute the cost-to-go between two configurations is available. 
% %along a collision-free trajectory generated by planner. The deep neural network learns cost-to-go functions for two input configurations given workspace conditions. 

%  Since the suggested network can learn cost-to-go function defined by any trajectory planner, it is applicable for high dimensional robot manipulator with random obstacles in workspace by training with planners operating in high dimensional space.

% Path planning for manipulators with obstacle avoidance requires heavy computation due to extensive collision checking with kinematics considerable iterative propagation of cost values. 
% In our suggestion, once the \ctog function is learned, the planner could generate a sub-optimal trajectory rapidly in a continuous configuration space while avoiding obstacle by following the gradient of \ctog function without intensive collision checks or iterative value computations.


% For scalar cost-to-go field of C-space $U: \mathcal{C} \rightarrow \mathbb {R}$, the cost-to-go value between $s$ and $t$ is the integral along a piecewise collision-free smooth curve $\mathbb {C} \subset \mathcal {C}$ is defined as,
% $$
% f_{\mathcal{W}}(s, t) = {\int _{\mathbb {C}}U(\mathbf {r} )\,ds=\int _{s}^{t}U\left(\mathbf {r} (t)\right)|\mathbf {r} '(t)|\,dt.}
% $$
% where $\mathbf {r} :[s,t]\rightarrow {\mathbb {C}}$  is an bijective parameterization of the curve $\mathcal {C}$ such that ${ \mathbf {r} (s)}$ and $ \mathbf {r} (t)$ give the endpoints of ${\mathbb {C}}$. 


\subsection{Method Overview}

The suggested network is trained via supervised learning to closely replicate \ctog values by Dijkstra in low dimensional space or by Probabilistic Roadmaps in high dimensional space. The network is trained to output a \ctog function of two configurations in C-space. 
However, since the collision space of C-space is changed according to conditions of workspace, the \ctog value is a function of two configurations given a workspace condition. It is difficult to learn a neural network for the cost-to-go values directly given workspace conditions due to sample complexity.  

We present an approach that the \ctog function is represented by one network and another network generates this continuous \ctog function network. The key idea of this approach is that once the workspace is encoded to the \ctog function network, \ctog is a function of only input configurations. During the training, the network generating the continuous \ctog function is trained to appropriately encode the workspace information for \ctog function network.

The network architecture used in this paper, we call \ours{}, consists of two components: (1)~HOF network which outputs the weights of the \ctog{} function from the workspace, and (2)~the \ctog{} function represented as a neural network which can map any two configurations to a positive real number which represents the distance of these configurations  (i.e., the \ctog{} value).

The first component is the HOF network which is trained to output the \ctog{} function (the weights of the \ctog network) from the input workspace $\mathcal{W}$ represented by pointcloud of obstacles.
The specific encoder used in this component depends on the representation of the $\mathcal{W}$. Since we use
pointcloud for representation of $\mathcal{W}$, we can apply PointNet ~\cite{qi2017pointnet} in this paper. For 2D image or 3D voxel of worksapce, we can apply image and voxel based convolution encoders. 
The second compoent is the c2g network which inputs two configurations and output is a value between two input configurations. The output of c2g network is a continuous value, and it is not directly linked to the input representation. This is because, during training, a denser set of samples continuously sampled from dataset are used to adjust the weights of the neural network representing the \ctog{} function . To summarize, the HOF encoder takes the pointcloud as input $\mathcal{W}$ and generates a \ctog{} function $f_w : \mathcal{Q} \times \mathcal{Q} \rightarrow \mathcal{C}$, such that  
for all $q_1, q_2 \in \mathcal{Q}$, 
$c = f_w(q_1, q_2) \in \mathcal{C}$ is the \ctog{} between $q_1$ and $q_2$. 

The difficulty of traditional planning based on \ctog estimation is that it requires computation of \ctog whenever it changes the environment and the goal point. For example, Dijkstra requires to compute the \ctog values whenever the goal is changed and it needs to reconstruct the connectivity among cells whenever the environment is changed for planing.
However, ours could compute the \ctog value with computational efficiency although workspace and the goal are changed,and  motion planning can be performed by following the gradient of \ctog to the goal point.
Another strength of this approach, it doesn't require encoding of the workspace if the environment is not changed, and we can use the compact c2g network for cost-go-values two pair points over the entire configuration space.

% modify ISER state estimation

%Compared to traditional approaches which requires discretization of space or has difficulty from curse of dimensionality, this approach is for rapid continuous motion planning in high dimensional space.


